ReSi: A Comprehensive Benchmark for Representational Similarity Measures

Measuring the similarity of different representations of neural architectures is a fundamental task and an open research challenge for the machine learning community. This paper presents the first comprehensive benchmark for evaluating representational similarity measures based on well-defined groundings of similarity. The representational similarity (ReSi) benchmark consists of (i) six carefully designed tests for similarity measures, (ii) 24 similarity measures, (iii) 14 neural network architectures, and (iv) seven datasets, spanning over the graph, language, and vision domains. The benchmark opens up several important avenues of research on representational similarity that enable novel explorations and applications of neural architectures. We demonstrate the utility of the ReSi benchmark by conducting experiments on various neural network architectures, real world datasets and similarity measures. All components of the benchmark are publicly available and thereby facilitate systematic reproduction and production of research results. The benchmark is extensible, future research can build on and further expand it. We believe that the ReSi benchmark can serve as a sound platform catalyzing future research that aims to systematically evaluate existing and explore novel ways of comparing representations of neural architectures.

==> tables/graphs_results_accuracy_correlation_test.tex <==
\begin{tabular}{l||rrrr|rrr|rrr||rrrr|rrr|rrr}
\toprule
Dataset & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} \\
Model & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT \\\rowcolor{Gray}
\midrule
AlignCos & -0.33 & 0.13 & -0.29 & -0.08 & 0.35 & 0.24 & -0.07 & -0.08 & 0.17 & -0.17 \\
CKA & 0.16 & -0.17 & 0.02 & -0.08 & 0.03 & 0.27 & -0.16 & -0.17 & 0.11 & -0.05 \\\rowcolor{Gray}
ConcDiff & 0.15 & -0.25 & -0.20 & 0.13 & -0.08 & -0.29 & -0.07 & -0.07 & -0.13 & -0.12 \\
DistCorr & 0.01 & -0.17 & 0.03 & 0.17 & 0.41 & \textbf{0.42} & -0.19 & -0.10 & 0.15 & -0.06 \\\rowcolor{Gray}
EOS & -0.24 & 0.08 & -0.05 & -0.04 & 0.15 & -0.27 & \textbf{0.29} & -0.21 & 0.05 & -0.32 \\
GULP & -0.43 & 0.08 & -0.12 & -0.02 & 0.04 & -0.27 & -0.27 & -0.08 & 0.06 & -0.34 \\\rowcolor{Gray}
HardCorr & 0.11 & -0.11 & -0.14 & -0.12 & 0.31 & 0.35 & 0.06 & \textbf{0.37} & 0.02 & 0.04 \\
IMD & -0.10 & 0.00 & -0.03 & 0.04 & -0.10 & 0.37 & -0.09 & -0.21 & -0.02 & -0.15 \\\rowcolor{Gray}
Jaccard & 0.02 & -0.11 & -0.16 & 0.07 & 0.32 & 0.28 & -0.18 & -0.32 & -0.13 & -0.14 \\
LinReg & 0.06 & -0.21 & -0.11 & -0.14 & -0.04 & 0.17 & -0.18 & 0.07 & -0.01 & -0.19 \\\rowcolor{Gray}
MagDiff & 0.08 & -0.13 & -0.19 & 0.18 & 0.02 & -0.17 & 0.14 & -0.18 & -0.20 & 0.11 \\
ShapeMet & 0.15 & -0.29 & -0.12 & -0.02 & 0.39 & 0.28 & -0.15 & -0.04 & 0.09 & -0.09 \\\rowcolor{Gray}
OrthProc & 0.15 & -0.29 & -0.12 & -0.02 & 0.39 & 0.28 & -0.15 & -0.04 & 0.09 & -0.09 \\
PWCCA & -0.05 & 0.07 & -0.26 & -0.09 & nan & -0.05 & -0.16 & -0.09 & 0.06 & -0.30 \\\rowcolor{Gray}
PermProc & -0.12 & \textbf{0.18} & -0.26 & 0.29 & 0.20 & -0.19 & 0.15 & -0.09 & 0.03 & 0.43 \\
ProcDist & 0.08 & 0.01 & -0.19 & \textbf{0.29} & 0.02 & -0.06 & 0.11 & -0.17 & 0.07 & \textbf{0.43} \\\rowcolor{Gray}
RSA & -0.27 & 0.04 & -0.28 & 0.21 & 0.53 & 0.32 & -0.08 & -0.07 & \textbf{0.25} & 0.32 \\
RSMDiff & -0.19 & 0.07 & -0.14 & 0.24 & -0.18 & -0.16 & 0.13 & -0.05 & -0.19 & 0.02 \\\rowcolor{Gray}
RankSim & -0.00 & -0.10 & \textbf{0.32} & 0.23 & 0.35 & 0.31 & -0.20 & -0.28 & 0.05 & -0.09 \\
SVCCA & -0.02 & -0.13 & -0.19 & -0.33 & 0.01 & 0.01 & -0.18 & -0.27 & 0.10 & -0.10 \\\rowcolor{Gray}
2nd-Cos & -0.10 & 0.04 & -0.11 & 0.13 & \textbf{0.54} & -0.19 & 0.01 & -0.47 & 0.22 & -0.19 \\
SoftCorr & \textbf{0.18} & -0.05 & 0.03 & -0.02 & 0.30 & 0.33 & -0.07 & 0.35 & 0.12 & 0.12 \\\rowcolor{Gray}
UnifDiff & -0.10 & -0.04 & -0.09 & -0.13 & -0.18 & 0.03 & -0.18 & -0.19 & -0.20 & -0.25 \\
\bottomrule
\end{tabular}


==> tables/graphs_results_augmentation_test.tex <==
\begin{tabular}{l||rrr|rrr|rrr||rrr|rrr|rrr}
\toprule
Measure & \multicolumn{9}{c}{AUPRC} & \multicolumn{9}{c}{Conformity Rate} \\
Dataset & \multicolumn{3}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} & \multicolumn{3}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} \\
Model & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT \\\rowcolor{Gray}
\midrule
AlignCos & 0.51 & 0.63 & 0.91 & 0.69 & 0.70 & 0.54 & 0.74 & 0.43 & \textbf{1.00} & 0.78 & 0.88 & 0.98 & 0.87 & 0.90 & 0.81 & 0.87 & 0.54 & \textbf{1.00} \\
CKA & 0.70 & 0.73 & 0.91 & 0.57 & 0.75 & 0.51 & 1.00 & \textbf{1.00} & 0.99 & 0.90 & 0.92 & 0.97 & 0.83 & 0.91 & 0.74 & 1.00 & \textbf{1.00} & 1.00 \\\rowcolor{Gray}
ConcDiff & 0.17 & 0.50 & 0.62 & 0.41 & 0.35 & 0.53 & 0.43 & 0.53 & 0.51 & 0.49 & 0.78 & 0.87 & 0.78 & 0.68 & 0.74 & 0.76 & 0.80 & 0.84 \\
DistCorr & 0.79 & 0.73 & 0.89 & 0.60 & 0.79 & 0.61 & \textbf{1.00} & \textbf{1.00} & 0.99 & 0.93 & 0.91 & 0.97 & 0.84 & 0.94 & 0.81 & \textbf{1.00} & \textbf{1.00} & 1.00 \\\rowcolor{Gray}
EOS & 0.53 & 0.62 & 0.34 & 0.68 & 0.53 & 0.46 & 0.82 & 0.49 & \textbf{1.00} & 0.86 & 0.90 & 0.75 & 0.88 & 0.80 & 0.70 & 0.96 & 0.75 & \textbf{1.00} \\
GULP & 0.45 & 0.61 & 0.35 & 0.22 & 0.54 & 0.55 & 0.56 & 0.48 & \textbf{1.00} & 0.79 & 0.89 & 0.76 & 0.52 & 0.81 & 0.84 & 0.80 & 0.75 & \textbf{1.00} \\\rowcolor{Gray}
HardCorr & 0.51 & 0.63 & 0.51 & 0.71 & 0.72 & 0.57 & 0.47 & 0.51 & 0.54 & 0.85 & 0.89 & 0.81 & 0.89 & 0.92 & \textbf{0.85} & 0.59 & 0.77 & 0.79 \\
IMD & 0.74 & 0.34 & 0.20 & 0.59 & 0.57 & 0.28 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.93 & 0.64 & 0.46 & 0.87 & 0.86 & 0.53 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
Jaccard & 0.78 & 0.81 & 0.95 & 0.74 & 0.88 & 0.58 & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.90 & 0.95 & 0.98 & 0.88 & 0.97 & 0.84 & \textbf{1.00} & 1.00 & \textbf{1.00} \\
LinReg & 0.94 & 0.85 & 0.87 & 0.30 & 0.81 & 0.34 & 0.72 & 0.72 & 0.81 & 0.98 & 0.96 & 0.95 & 0.53 & 0.93 & 0.69 & 0.83 & 0.83 & 0.93 \\\rowcolor{Gray}
MagDiff & 0.20 & 0.39 & 0.54 & 0.59 & 0.17 & 0.43 & 0.77 & \textbf{1.00} & 0.69 & 0.51 & 0.74 & 0.83 & 0.87 & 0.45 & 0.66 & 0.93 & \textbf{1.00} & 0.91 \\
ShapeMet & 0.81 & 0.78 & 0.83 & 0.63 & 0.76 & 0.54 & 0.72 & 0.72 & 0.74 & 0.95 & 0.93 & 0.95 & 0.85 & 0.94 & 0.77 & 0.83 & 0.83 & 0.89 \\\rowcolor{Gray}
OrthProc & 0.81 & 0.78 & 0.83 & 0.63 & 0.76 & 0.54 & 0.72 & 0.72 & 0.74 & 0.95 & 0.93 & 0.95 & 0.85 & 0.94 & 0.77 & 0.83 & 0.83 & 0.89 \\
PWCCA & 0.60 & 0.65 & 0.42 & nan & 0.57 & 0.51 & nan & 0.48 & 0.82 & 0.86 & 0.89 & 0.83 & nan & 0.83 & 0.75 & nan & 0.74 & 0.96 \\\rowcolor{Gray}
PermProc & 0.70 & 0.61 & 0.42 & 0.65 & 0.69 & 0.40 & 0.88 & 0.73 & 0.94 & 0.78 & 0.89 & 0.51 & 0.87 & 0.90 & 0.62 & 0.97 & 0.87 & 0.98 \\
ProcDist & 0.76 & 0.69 & 0.75 & 0.70 & 0.81 & 0.40 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.88 & 0.90 & 0.90 & 0.89 & 0.95 & 0.63 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
RSA & 0.39 & 0.57 & 0.78 & 0.68 & 0.72 & 0.59 & 0.75 & 0.49 & 0.67 & 0.68 & 0.84 & 0.94 & 0.86 & 0.92 & 0.84 & 0.89 & 0.78 & 0.85 \\
RSMDiff & \textbf{0.99} & 0.79 & \textbf{1.00} & 0.64 & \textbf{0.93} & 0.40 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.93 & \textbf{1.00} & 0.87 & 0.97 & 0.62 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
RankSim & 0.54 & 0.62 & 0.95 & 0.75 & 0.88 & 0.55 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.72 & 0.88 & 0.98 & 0.89 & 0.96 & 0.83 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
SVCCA & 0.27 & 0.29 & 0.34 & 0.64 & 0.67 & 0.49 & 0.89 & 0.81 & 0.82 & 0.54 & 0.55 & 0.58 & 0.84 & 0.86 & 0.68 & 0.89 & 0.85 & 0.91 \\\rowcolor{Gray}
2nd-Cos & 0.73 & \textbf{0.86} & 0.97 & \textbf{0.78} & 0.92 & \textbf{0.62} & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.88 & \textbf{0.97} & 0.99 & \textbf{0.91} & \textbf{0.98} & 0.84 & \textbf{1.00} & 1.00 & \textbf{1.00} \\
SoftCorr & 0.63 & 0.70 & 0.50 & 0.73 & 0.58 & 0.55 & 0.43 & 0.46 & 0.45 & 0.89 & 0.92 & 0.80 & 0.87 & 0.85 & 0.84 & 0.51 & 0.71 & 0.66 \\\rowcolor{Gray}
UnifDiff & 0.75 & 0.53 & \textbf{1.00} & 0.68 & 0.24 & 0.25 & 0.76 & 0.53 & 0.45 & 0.91 & 0.86 & \textbf{1.00} & 0.90 & 0.52 & 0.66 & 0.88 & 0.81 & 0.78 \\
\bottomrule
\end{tabular}


==> tables/graphs_results_label_test.tex <==
\begin{tabular}{l||rrrr|rrr|rrr||rrrr|rrr|rrr}
\toprule
Measure & \multicolumn{10}{c}{AUPRC} & \multicolumn{10}{c}{Conformity Rate} \\
Dataset & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} \\
Model & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT \\\rowcolor{Gray}
\midrule
AlignCos & 0.46 & 0.48 & 0.43 & 0.23 & 0.84 & 0.42 & 0.29 & 0.98 & 0.70 & 0.93 & 0.66 & 0.66 & 0.60 & 0.60 & 0.94 & 0.50 & 0.58 & 1.00 & 0.67 & 0.97 \\
CKA & 0.43 & 0.42 & 0.42 & 0.24 & 0.73 & 0.66 & 0.27 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.55 & 0.51 & 0.51 & 0.58 & 0.91 & 0.86 & 0.54 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
ConcDiff & 0.20 & 0.39 & 0.39 & 0.18 & 0.37 & 0.57 & 0.21 & 0.96 & \textbf{1.00} & 1.00 & 0.54 & 0.78 & 0.74 & 0.46 & 0.72 & 0.85 & 0.48 & 0.99 & \textbf{1.00} & 1.00 \\
DistCorr & 0.43 & 0.44 & 0.42 & 0.25 & 0.86 & 0.43 & 0.22 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.59 & 0.63 & 0.52 & \textbf{0.66} & 0.95 & 0.56 & 0.52 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
EOS & 0.30 & 0.26 & 0.28 & 0.26 & 0.41 & 0.42 & 0.22 & 0.25 & 0.43 & 0.34 & 0.65 & 0.55 & 0.66 & 0.58 & 0.50 & 0.52 & 0.58 & 0.50 & 0.54 & 0.51 \\
GULP & 0.28 & 0.26 & 0.28 & 0.26 & 0.19 & 0.42 & 0.23 & 0.30 & 0.43 & 0.30 & 0.63 & 0.56 & 0.66 & 0.54 & 0.50 & 0.51 & 0.57 & 0.49 & 0.55 & 0.56 \\\rowcolor{Gray}
HardCorr & 0.42 & 0.42 & 0.42 & 0.21 & 0.77 & 0.46 & 0.33 & 0.83 & 0.83 & 0.54 & 0.53 & 0.51 & 0.51 & 0.54 & 0.94 & 0.68 & 0.67 & 0.97 & 0.97 & 0.77 \\
IMD & \textbf{0.73} & \textbf{0.97} & \textbf{0.84} & 0.23 & 0.24 & 0.37 & 0.23 & \textbf{1.00} & \textbf{1.00} & 0.90 & \textbf{0.93} & \textbf{0.99} & \textbf{0.96} & 0.54 & 0.47 & 0.70 & 0.54 & \textbf{1.00} & \textbf{1.00} & 0.97 \\\rowcolor{Gray}
Jaccard & 0.42 & 0.42 & 0.43 & 0.24 & 0.56 & 0.43 & 0.29 & 0.83 & 0.43 & 0.78 & 0.53 & 0.51 & 0.55 & 0.57 & 0.77 & 0.58 & 0.57 & 0.97 & 0.53 & 0.93 \\
LinReg & 0.49 & 0.43 & 0.46 & 0.24 & 0.22 & 0.45 & 0.23 & 0.44 & 0.68 & 0.47 & 0.71 & 0.58 & 0.69 & 0.54 & 0.49 & 0.66 & 0.52 & 0.63 & 0.81 & 0.63 \\\rowcolor{Gray}
MagDiff & 0.20 & 0.24 & 0.37 & 0.28 & 0.66 & 0.72 & 0.18 & 0.55 & 0.49 & 0.34 & 0.51 & 0.60 & 0.74 & 0.61 & 0.89 & 0.93 & 0.47 & 0.83 & 0.86 & 0.75 \\
ShapeMet & 0.43 & 0.42 & 0.42 & 0.23 & \textbf{0.88} & 0.43 & 0.27 & 0.83 & 0.73 & 0.77 & 0.54 & 0.51 & 0.52 & 0.60 & \textbf{0.95} & 0.60 & 0.53 & 0.97 & 0.84 & 0.88 \\\rowcolor{Gray}
OrthProc & 0.43 & 0.42 & 0.42 & 0.23 & \textbf{0.88} & 0.43 & 0.27 & 0.83 & 0.73 & 0.77 & 0.54 & 0.51 & 0.52 & 0.60 & \textbf{0.95} & 0.60 & 0.53 & 0.97 & 0.84 & 0.88 \\
PWCCA & 0.26 & 0.33 & 0.28 & 0.25 & nan & 0.44 & 0.24 & 0.24 & 0.44 & 0.36 & 0.60 & 0.52 & 0.64 & 0.58 & nan & 0.64 & 0.53 & 0.43 & 0.61 & 0.56 \\\rowcolor{Gray}
PermProc & 0.44 & 0.39 & 0.44 & 0.27 & 0.77 & 0.90 & 0.19 & 0.68 & 0.72 & 0.93 & 0.64 & 0.71 & 0.61 & 0.52 & 0.94 & 0.97 & 0.50 & 0.84 & 0.88 & 0.98 \\
ProcDist & 0.45 & 0.45 & 0.43 & 0.27 & 0.79 & 0.62 & 0.19 & 0.92 & 0.98 & \textbf{1.00} & 0.67 & 0.68 & 0.60 & 0.51 & 0.93 & 0.88 & 0.51 & 0.98 & 1.00 & \textbf{1.00} \\\rowcolor{Gray}
RSA & 0.46 & 0.44 & 0.43 & 0.23 & 0.74 & 0.42 & 0.33 & 0.96 & 0.43 & 0.49 & 0.69 & 0.61 & 0.54 & 0.58 & 0.89 & 0.52 & 0.64 & 0.99 & 0.58 & 0.63 \\
RSMDiff & 0.52 & 0.53 & 0.78 & \textbf{0.29} & 0.71 & \textbf{0.92} & 0.19 & 1.00 & \textbf{1.00} & \textbf{1.00} & 0.73 & 0.83 & 0.86 & 0.61 & 0.91 & \textbf{0.97} & 0.51 & 1.00 & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
RankSim & 0.45 & 0.42 & 0.47 & 0.22 & 0.47 & 0.43 & 0.33 & 0.84 & 0.55 & 0.78 & 0.65 & 0.54 & 0.64 & 0.54 & 0.66 & 0.53 & 0.58 & 0.97 & 0.63 & 0.93 \\
SVCCA & 0.35 & 0.31 & 0.42 & 0.20 & 0.33 & 0.80 & 0.27 & \textbf{1.00} & \textbf{1.00} & 0.93 & 0.62 & 0.56 & 0.59 & 0.39 & 0.69 & 0.91 & 0.54 & \textbf{1.00} & \textbf{1.00} & 0.96 \\\rowcolor{Gray}
2nd-Cos & 0.56 & 0.73 & 0.73 & 0.21 & 0.61 & 0.42 & 0.36 & 0.99 & 0.96 & 0.95 & 0.80 & 0.87 & 0.86 & 0.51 & 0.82 & 0.50 & 0.66 & 1.00 & 0.99 & 0.99 \\
SoftCorr & 0.42 & 0.42 & 0.42 & 0.23 & 0.60 & 0.45 & 0.33 & 0.83 & 0.82 & 0.55 & 0.53 & 0.51 & 0.50 & 0.55 & 0.85 & 0.67 & 0.65 & 0.97 & 0.96 & 0.71 \\\rowcolor{Gray}
UnifDiff & 0.33 & 0.50 & 0.32 & 0.29 & 0.53 & 0.90 & \textbf{0.40} & 0.53 & 0.54 & 0.33 & 0.70 & 0.81 & 0.67 & 0.59 & 0.84 & 0.96 & \textbf{0.75} & 0.78 & 0.81 & 0.66 \\
\bottomrule
\end{tabular}


==> tables/graphs_results_layer_test.tex <==
\begin{tabular}{l||rrrr|rrr|rrr||rrrr|rrr|rrr}
\toprule
Measure & \multicolumn{10}{c}{Spearman Correlation} & \multicolumn{10}{c}{Conformity Rate} \\
Dataset & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} \\
Model & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT \\\rowcolor{Gray}
\midrule
AlignCos & 0.98 & \textbf{1.00} & \textbf{1.00} & 0.45 & 0.33 & 0.68 & 0.04 & 0.84 & 0.93 & 0.84 & 0.97 & \textbf{1.00} & \textbf{1.00} & 0.64 & 0.59 & 0.77 & 0.46 & 0.83 & 0.93 & 0.89 \\
CKA & 0.98 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.60 & 0.89 & 0.39 & 0.85 & 0.46 & 0.96 & 0.98 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.79 & 0.92 & 0.59 & 0.87 & 0.64 & 0.95 \\\rowcolor{Gray}
ConcDiff & 0.85 & 0.25 & 0.40 & 0.14 & 0.38 & -0.27 & 0.24 & 0.73 & 0.39 & 0.40 & 0.85 & 0.52 & 0.62 & 0.52 & 0.57 & 0.36 & 0.58 & 0.70 & 0.74 & 0.67 \\
DistCorr & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.93 & 0.63 & 0.99 & 0.47 & 0.81 & 0.52 & 0.93 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.99 & 0.81 & 0.99 & 0.63 & 0.88 & 0.65 & 0.92 \\\rowcolor{Gray}
EOS & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.92 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.98 & \textbf{1.00} & \textbf{1.00} & 0.92 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
GULP & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.82 & 0.54 & \textbf{1.00} & 0.33 & 0.73 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.90 & 0.83 & \textbf{1.00} & 0.72 & 0.82 & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
HardCorr & 0.83 & 0.98 & 0.54 & 0.82 & 0.63 & 0.80 & 0.21 & 0.83 & 0.62 & \textbf{1.00} & 0.91 & 0.99 & 0.76 & 0.85 & 0.81 & 0.84 & 0.68 & 0.86 & 0.72 & \textbf{1.00} \\
IMD & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.89 & \textbf{1.00} & 0.82 & 0.97 & 0.55 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.95 & \textbf{1.00} & 0.94 & 0.97 & 0.85 & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
Jaccard & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.95 & 0.97 & 0.95 & 0.97 & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.94 & 0.96 & 0.96 & 0.96 & 0.98 & \textbf{1.00} \\
LinReg & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.45 & \textbf{1.00} & 0.03 & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.95 & 0.67 & \textbf{1.00} & 0.59 & 0.99 & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
MagDiff & 0.55 & 0.49 & 0.89 & 0.91 & 0.58 & 0.50 & 0.38 & 0.06 & 0.29 & 0.63 & 0.63 & 0.72 & 0.92 & 0.97 & 0.65 & 0.63 & 0.58 & 0.52 & 0.71 & 0.87 \\
ShapeMet & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.91 & 0.62 & 0.98 & 0.45 & 0.97 & 0.99 & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.97 & 0.80 & 0.99 & 0.66 & 0.95 & 0.99 & 0.99 \\\rowcolor{Gray}
OrthProc & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.91 & 0.62 & 0.98 & 0.45 & 0.97 & 0.99 & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.97 & 0.80 & 0.99 & 0.66 & 0.95 & 0.99 & 0.99 \\
PWCCA & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & nan & \textbf{1.00} & 0.37 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.75 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
PermProc & 0.92 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.60 & 0.68 & 0.63 & 0.24 & 0.88 & \textbf{1.00} & 0.91 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.68 & 0.72 & 0.75 & 0.69 & 0.87 & \textbf{1.00} \\
ProcDist & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.91 & 0.66 & \textbf{1.00} & 0.62 & 0.83 & 0.85 & \textbf{1.00} & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.97 & 0.75 & \textbf{1.00} & 0.78 & 0.93 & 0.96 & \textbf{1.00} \\\rowcolor{Gray}
RSA & 0.84 & 0.91 & \textbf{1.00} & 0.52 & 0.58 & 0.99 & 0.44 & 0.52 & 0.97 & 0.94 & 0.90 & 0.97 & \textbf{1.00} & 0.72 & 0.70 & 0.98 & 0.70 & 0.81 & 0.97 & 0.94 \\
RSMDiff & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.91 & 0.54 & 0.65 & 0.81 & 0.85 & 0.93 & \textbf{1.00} & 0.99 & \textbf{1.00} & \textbf{1.00} & 0.97 & 0.66 & 0.68 & 0.92 & 0.85 & 0.93 & \textbf{1.00} \\\rowcolor{Gray}
RankSim & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.99 & 0.95 & 0.97 & \textbf{0.99} & 0.99 & 0.99 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.99 & 0.94 & 0.95 & \textbf{0.98} & 0.99 & 0.98 & \textbf{1.00} \\
SVCCA & 0.41 & 0.78 & 0.61 & \textbf{1.00} & 0.53 & 0.44 & 0.47 & -0.17 & -0.10 & 0.33 & 0.63 & 0.80 & 0.81 & \textbf{1.00} & 0.75 & 0.69 & 0.57 & 0.49 & 0.41 & 0.56 \\\rowcolor{Gray}
2nd-Cos & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.92 & 0.81 & 0.96 & 0.52 & 0.97 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.92 & 0.91 & 0.96 & 0.67 & 0.95 & \textbf{1.00} & \textbf{1.00} \\
SoftCorr & 0.96 & 0.99 & 0.50 & 0.74 & 0.79 & 0.89 & 0.11 & 0.91 & 0.62 & \textbf{1.00} & 0.95 & 0.99 & 0.78 & 0.82 & 0.89 & 0.88 & 0.64 & 0.91 & 0.73 & \textbf{1.00} \\\rowcolor{Gray}
UnifDiff & 0.67 & 0.67 & 0.59 & 0.56 & 0.82 & 0.89 & 0.82 & 0.33 & -0.45 & 0.68 & 0.70 & 0.70 & 0.69 & 0.69 & 0.94 & 0.92 & 0.94 & 0.60 & 0.41 & 0.83 \\
\bottomrule
\end{tabular}


==> tables/graphs_results_output_correlation_test.tex <==
\begin{tabular}{l||rrrr|rrr|rrr||rrrr|rrr|rrr}
\toprule
Measure & \multicolumn{10}{c}{Disagreement} & \multicolumn{10}{c}{JSD} \\
Dataset & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} \\
Model & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT \\\rowcolor{Gray}
\midrule
AlignCos & -0.08 & 0.27 & -0.05 & 0.01 & 0.15 & 0.37 & -0.08 & -0.10 & 0.00 & 0.17 & 0.02 & 0.38 & 0.17 & -0.15 & 0.31 & 0.44 & -0.01 & -0.03 & 0.05 & 0.28 \\
CKA & 0.36 & 0.00 & 0.45 & 0.07 & -0.21 & 0.53 & 0.06 & 0.03 & -0.04 & 0.23 & 0.43 & -0.03 & 0.53 & -0.25 & 0.03 & 0.58 & 0.17 & 0.12 & -0.02 & 0.38 \\\rowcolor{Gray}
ConcDiff & -0.04 & -0.10 & 0.03 & 0.13 & -0.21 & -0.04 & 0.03 & -0.25 & 0.07 & -0.16 & 0.03 & 0.04 & 0.01 & \textbf{0.34} & -0.17 & -0.03 & 0.03 & -0.13 & 0.02 & -0.22 \\
DistCorr & 0.53 & -0.08 & \textbf{0.46} & 0.10 & 0.17 & 0.40 & -0.03 & 0.11 & 0.08 & 0.20 & 0.60 & 0.05 & \textbf{0.60} & -0.28 & 0.46 & 0.43 & 0.03 & 0.16 & 0.12 & 0.36 \\\rowcolor{Gray}
EOS & 0.13 & 0.02 & -0.09 & 0.17 & 0.02 & 0.33 & \textbf{0.23} & -0.25 & -0.02 & 0.12 & 0.17 & 0.22 & -0.04 & -0.26 & -0.03 & 0.38 & 0.11 & -0.17 & 0.11 & 0.37 \\
GULP & -0.17 & -0.09 & -0.13 & \textbf{0.53} & 0.03 & 0.33 & -0.01 & 0.15 & -0.04 & 0.10 & -0.10 & 0.18 & -0.04 & 0.19 & 0.15 & 0.38 & 0.13 & 0.10 & 0.11 & 0.35 \\\rowcolor{Gray}
HardCorr & 0.45 & 0.10 & 0.26 & 0.27 & \textbf{0.40} & 0.46 & -0.09 & 0.02 & -0.24 & 0.24 & 0.48 & 0.16 & 0.52 & -0.15 & \textbf{0.53} & 0.50 & 0.09 & -0.05 & -0.28 & 0.46 \\
IMD & 0.20 & -0.11 & -0.13 & 0.01 & -0.10 & 0.33 & -0.02 & -0.13 & 0.01 & 0.04 & 0.24 & -0.38 & -0.09 & 0.05 & -0.08 & 0.29 & 0.04 & -0.13 & -0.03 & 0.01 \\\rowcolor{Gray}
Jaccard & 0.44 & 0.33 & 0.12 & 0.24 & 0.04 & 0.42 & -0.00 & 0.14 & 0.01 & 0.22 & 0.44 & 0.45 & 0.38 & -0.02 & 0.33 & 0.42 & 0.11 & 0.20 & 0.09 & 0.37 \\
LinReg & 0.57 & 0.09 & -0.06 & 0.10 & 0.12 & 0.46 & 0.06 & -0.10 & -0.19 & 0.22 & 0.58 & 0.33 & 0.19 & -0.27 & 0.15 & 0.48 & 0.18 & -0.09 & -0.17 & 0.47 \\\rowcolor{Gray}
MagDiff & -0.07 & -0.25 & -0.07 & 0.36 & 0.06 & 0.07 & -0.20 & -0.25 & -0.19 & 0.22 & 0.00 & 0.06 & -0.15 & 0.24 & 0.03 & 0.06 & -0.26 & -0.13 & -0.13 & 0.08 \\
ShapeMet & \textbf{0.62} & 0.16 & 0.05 & 0.20 & 0.19 & 0.57 & 0.03 & 0.02 & -0.16 & 0.27 & \textbf{0.70} & 0.27 & 0.28 & -0.15 & 0.43 & 0.63 & 0.13 & 0.04 & -0.15 & 0.44 \\\rowcolor{Gray}
OrthProc & \textbf{0.62} & 0.16 & 0.05 & 0.20 & 0.19 & 0.57 & 0.03 & 0.02 & -0.16 & 0.27 & \textbf{0.70} & 0.27 & 0.28 & -0.15 & 0.43 & 0.63 & 0.13 & 0.04 & -0.15 & 0.44 \\
PWCCA & 0.08 & \textbf{0.36} & -0.14 & 0.06 & nan & 0.32 & 0.16 & -0.24 & -0.08 & 0.03 & 0.08 & 0.27 & 0.02 & -0.37 & nan & 0.38 & \textbf{0.27} & -0.22 & -0.04 & 0.29 \\\rowcolor{Gray}
PermProc & 0.24 & 0.33 & -0.14 & 0.46 & 0.18 & -0.10 & -0.27 & 0.25 & -0.41 & 0.22 & 0.29 & 0.10 & 0.13 & 0.22 & 0.29 & -0.10 & -0.42 & 0.34 & -0.55 & 0.06 \\
ProcDist & 0.45 & 0.24 & -0.17 & 0.46 & -0.13 & -0.15 & -0.27 & \textbf{0.26} & -0.38 & 0.30 & 0.52 & 0.08 & 0.05 & 0.22 & 0.02 & -0.18 & -0.38 & \textbf{0.36} & -0.50 & 0.13 \\\rowcolor{Gray}
RSA & 0.06 & 0.33 & -0.02 & 0.38 & 0.35 & \textbf{0.59} & 0.06 & 0.17 & 0.15 & \textbf{0.45} & 0.12 & 0.13 & 0.20 & 0.21 & 0.52 & \textbf{0.63} & 0.14 & 0.20 & 0.14 & 0.46 \\
RSMDiff & 0.05 & 0.14 & -0.15 & 0.43 & -0.30 & -0.00 & -0.26 & -0.14 & 0.09 & 0.36 & 0.11 & -0.01 & -0.07 & 0.18 & -0.22 & -0.04 & -0.37 & -0.20 & 0.11 & 0.33 \\\rowcolor{Gray}
RankSim & 0.34 & 0.23 & 0.44 & 0.24 & 0.06 & 0.24 & 0.05 & 0.03 & \textbf{0.27} & 0.10 & 0.36 & \textbf{0.56} & 0.51 & 0.06 & 0.33 & 0.30 & 0.21 & 0.02 & \textbf{0.36} & 0.13 \\
SVCCA & -0.06 & 0.04 & 0.17 & 0.02 & -0.27 & 0.21 & 0.03 & 0.08 & 0.11 & -0.15 & -0.09 & 0.02 & 0.26 & -0.06 & -0.04 & 0.23 & 0.13 & 0.19 & 0.16 & -0.17 \\\rowcolor{Gray}
2nd-Cos & 0.40 & 0.25 & 0.30 & 0.02 & 0.30 & 0.14 & -0.10 & 0.04 & 0.27 & 0.06 & 0.43 & 0.54 & 0.53 & -0.19 & 0.47 & 0.15 & 0.07 & 0.11 & 0.34 & 0.11 \\
SoftCorr & 0.49 & 0.06 & 0.07 & 0.23 & 0.39 & 0.49 & 0.02 & 0.03 & -0.26 & 0.35 & 0.53 & -0.01 & 0.21 & -0.13 & 0.53 & 0.53 & 0.23 & 0.02 & -0.28 & \textbf{0.56} \\\rowcolor{Gray}
UnifDiff & 0.07 & 0.16 & -0.15 & 0.15 & -0.34 & 0.04 & 0.18 & -0.33 & 0.10 & 0.06 & 0.13 & 0.27 & -0.11 & -0.20 & -0.32 & 0.02 & 0.21 & -0.34 & 0.12 & 0.12 \\
\bottomrule
\end{tabular}


==> tables/graphs_results_shortcut_test.tex <==
\begin{tabular}{l||rrrr|rrr|rrr||rrrr|rrr|rrr}
\toprule
\cellcolor{white}Measure & \multicolumn{10}{c}{AUPRC} & \multicolumn{10}{c}{Conformity Rate} \\
Dataset & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} & \multicolumn{4}{c}{Cora} & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{OGBN-Arxiv} \\
Model & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT & GCN & SAGE & GAT & PGNN & GCN & SAGE & GAT & GCN & SAGE & GAT \\\rowcolor{Gray}
\midrule
AlignCos & 0.64 & 0.60 & 0.59 & 0.40 & 0.89 & \textbf{1.00} & 0.48 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.84 & 0.88 & 0.89 & 0.63 & 0.98 & \textbf{1.00} & 0.77 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
CKA & 0.61 & 0.78 & 0.78 & 0.34 & 0.28 & \textbf{1.00} & 0.33 & \textbf{1.00} & 0.98 & \textbf{1.00} & 0.75 & 0.90 & 0.94 & 0.63 & 0.57 & \textbf{1.00} & 0.65 & \textbf{1.00} & 1.00 & \textbf{1.00} \\\rowcolor{Gray}
ConcDiff & 0.51 & 0.17 & 0.20 & 0.17 & 0.18 & 0.18 & 0.32 & 0.81 & 0.96 & \textbf{1.00} & 0.77 & 0.43 & 0.54 & 0.44 & 0.50 & 0.46 & 0.61 & 0.96 & 0.99 & \textbf{1.00} \\
DistCorr & 0.66 & 0.82 & 0.80 & 0.42 & 0.33 & \textbf{1.00} & 0.32 & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.83 & 0.92 & 0.95 & 0.62 & 0.69 & \textbf{1.00} & 0.72 & \textbf{1.00} & 1.00 & \textbf{1.00} \\\rowcolor{Gray}
EOS & 0.30 & 0.50 & 0.20 & 0.37 & 0.46 & 0.43 & 0.54 & \textbf{1.00} & 0.72 & 0.97 & 0.71 & 0.74 & 0.46 & 0.50 & 0.87 & 0.60 & 0.81 & \textbf{1.00} & 0.83 & 0.99 \\
GULP & 0.31 & 0.50 & 0.20 & 0.37 & 0.20 & 0.43 & 0.45 & 0.99 & 0.72 & 0.96 & 0.72 & 0.74 & 0.46 & 0.50 & 0.49 & 0.60 & 0.81 & 1.00 & 0.83 & 0.99 \\\rowcolor{Gray}
HardCorr & 0.28 & 0.35 & 0.29 & 0.35 & 0.55 & \textbf{1.00} & 0.52 & 0.80 & 0.72 & 0.83 & 0.65 & 0.77 & 0.70 & 0.69 & 0.83 & \textbf{1.00} & 0.81 & 0.96 & 0.83 & 0.97 \\
IMD & 0.71 & 0.82 & 0.60 & 0.25 & 0.78 & 0.97 & 0.36 & 0.61 & 0.92 & 0.92 & 0.92 & 0.96 & 0.88 & 0.68 & 0.94 & 0.99 & 0.62 & 0.84 & 0.98 & 0.97 \\\rowcolor{Gray}
Jaccard & 0.74 & 0.78 & \textbf{0.86} & 0.42 & \textbf{1.00} & 0.83 & 0.54 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.91 & 0.93 & \textbf{0.97} & 0.53 & \textbf{1.00} & 0.96 & \textbf{0.84} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
LinReg & 0.70 & 0.74 & 0.50 & 0.34 & 0.37 & 0.61 & 0.36 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.88 & 0.95 & 0.75 & 0.62 & 0.70 & 0.81 & 0.72 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
MagDiff & 0.37 & 0.15 & 0.18 & 0.21 & 0.27 & 0.78 & 0.20 & 0.55 & 0.53 & \textbf{1.00} & 0.74 & 0.41 & 0.49 & 0.58 & 0.67 & 0.89 & 0.48 & 0.82 & 0.82 & \textbf{1.00} \\
ShapeMet & 0.63 & 0.79 & 0.62 & 0.35 & 0.58 & \textbf{1.00} & 0.31 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.79 & 0.91 & 0.90 & 0.63 & 0.80 & \textbf{1.00} & 0.72 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
OrthProc & 0.63 & 0.79 & 0.62 & 0.35 & 0.58 & \textbf{1.00} & 0.31 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.79 & 0.91 & 0.90 & 0.63 & 0.80 & \textbf{1.00} & 0.72 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
PWCCA & 0.33 & 0.47 & 0.22 & 0.38 & nan & 0.43 & 0.33 & 0.99 & 0.72 & 1.00 & 0.73 & 0.71 & 0.56 & 0.50 & nan & 0.60 & 0.73 & 1.00 & 0.83 & 1.00 \\\rowcolor{Gray}
PermProc & 0.23 & 0.27 & 0.25 & 0.25 & 0.42 & \textbf{1.00} & 0.27 & 0.65 & 0.43 & 0.77 & 0.57 & 0.67 & 0.64 & 0.57 & 0.72 & \textbf{1.00} & 0.58 & 0.86 & 0.60 & 0.91 \\
ProcDist & 0.60 & 0.81 & 0.68 & 0.25 & 0.60 & \textbf{1.00} & 0.33 & \textbf{1.00} & 1.00 & \textbf{1.00} & 0.77 & 0.91 & 0.92 & 0.58 & 0.82 & \textbf{1.00} & 0.61 & \textbf{1.00} & 1.00 & \textbf{1.00} \\\rowcolor{Gray}
RSA & 0.49 & 0.43 & 0.73 & 0.42 & 0.89 & \textbf{1.00} & 0.52 & 0.97 & 0.98 & 0.90 & 0.72 & 0.78 & 0.91 & \textbf{0.70} & 0.97 & \textbf{1.00} & 0.81 & 0.99 & 0.99 & 0.98 \\
RSMDiff & 0.46 & 0.50 & 0.69 & 0.37 & 0.48 & 0.92 & 0.36 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.70 & 0.76 & 0.91 & 0.64 & 0.75 & 0.97 & 0.59 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\rowcolor{Gray}
RankSim & 0.73 & 0.64 & 0.85 & \textbf{0.43} & \textbf{1.00} & 0.77 & 0.54 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 0.87 & 0.89 & 0.95 & 0.58 & \textbf{1.00} & 0.92 & 0.83 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
SVCCA & 0.23 & 0.36 & 0.46 & 0.24 & 0.24 & 0.93 & 0.32 & \textbf{1.00} & 0.97 & 0.83 & 0.46 & 0.60 & 0.69 & 0.52 & 0.57 & 0.97 & 0.66 & \textbf{1.00} & 0.99 & 0.91 \\\rowcolor{Gray}
2nd-Cos & \textbf{0.85} & \textbf{0.91} & 0.81 & 0.34 & \textbf{1.00} & \textbf{1.00} & 0.52 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{0.95} & \textbf{0.97} & 0.95 & 0.68 & \textbf{1.00} & \textbf{1.00} & 0.82 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
SoftCorr & 0.31 & 0.40 & 0.30 & 0.39 & 0.66 & \textbf{1.00} & \textbf{0.57} & 0.82 & 0.72 & 0.83 & 0.68 & 0.79 & 0.71 & 0.67 & 0.87 & \textbf{1.00} & 0.82 & 0.96 & 0.83 & 0.97 \\\rowcolor{Gray}
UnifDiff & 0.30 & 0.64 & 0.71 & 0.29 & 0.59 & 0.50 & 0.48 & 0.99 & 0.72 & 0.97 & 0.62 & 0.91 & 0.91 & 0.65 & 0.83 & 0.77 & 0.67 & 1.00 & 0.86 & 0.99 \\
\bottomrule
\end{tabular}


==> tables/layerdist_similarity_correlation_nlp.tex <==
\begin{table}[]
    \caption{Spearman rank correlation between distance of layers and representational similarity on the MNLI matched validation set (left) and SST2 test set (right) for a finetuned BERT model. 
    The embedding layer is excluded.
    All measures use preprocessing, such that they have OT,IS,TR invariance.
    }
    \label{tab:corr_layerdist_repsim_nlp}
    \centering
    \begin{tabular}{lcc}
\toprule
Measure & Median & Mean \\
\midrule
Aligned Cosine Similarity & 1.00 & 1.00 \\
Jaccard Similarity & 1.00 & 1.00 \\
Joint Rank-Jaccard Similarity & 1.00 & 1.00 \\
Orthogonal Procrustes & 1.00 & 1.00 \\
Distance Correlation & 1.00 & 1.00 \\
CKA & 1.00 & 1.00 \\
RSA (Euc,Spearman) & 1.00 & 1.00 \\
Norm of RSM Difference (Euc) & 1.00 & 0.99 \\
Second Order Cosine Similarity & 1.00 & 0.98 \\
Uniformity Difference & 0.98 & 0.94 \\
Rank Similarity & 0.99 & 0.77 \\
Magnitude Difference & 0.80 & 0.60 \\
Concentricity Difference & 0.10 & 0.19 \\
\bottomrule
\end{tabular}
\begin{tabular}{lcc}
\toprule
Measure & Median & Mean \\
\midrule
Aligned Cosine Similarity & 1.00 & 1.00 \\
Jaccard Similarity & 1.00 & 1.00 \\
Orthogonal Procrustes & 1.00 & 1.00 \\
Rank Similarity & 1.00 & 1.00 \\
RSA (Euc,Spearman) & 1.00 & 1.00 \\
Joint Rank-Jaccard Similarity & 1.00 & 1.00 \\
Norm of RSM Difference (Euc) & 1.00 & 0.99 \\
Distance Correlation & 1.00 & 0.99 \\
CKA & 1.00 & 0.95 \\
Second Order Cosine Similarity & 0.98 & 0.95 \\
Uniformity Difference & 0.98 & 0.94 \\
Magnitude Difference & 0.74 & 0.53 \\
Concentricity Difference & 0.38 & 0.24 \\
\bottomrule
\end{tabular}
    
\end{table}

==> tables/nlp_everything.tex <==
\begin{table}[h]
\caption{Results of Tests 1-6 for the language domain. %In all cases, we used BERT models.
}
\label{tab:nlp_results}
\resizebox{\linewidth}{!}{
\begin{tabular}{l||rr|rr|rr||rr|rr|rr|rr|rr|rr|rr|rr}
\toprule
Type & \multicolumn{6}{c}{Grounding by Prediction} & \multicolumn{16}{c}{Grounding by Design} \\
% Test & \multicolumn{2}{c}{Acc. Corr.} & \multicolumn{2}{c}{JSD Corr.} & \multicolumn{2}{c}{Disagr. Corr.} & \multicolumn{4}{c}{Label Randomization} & \multicolumn{4}{c}{Shortcut Affinity} & \multicolumn{4}{c}{Augmentation} & \multicolumn{4}{c}{Layer Monotonicity} \\
Test & \multicolumn{2}{c}{Corr. Acc. Diff.} & \multicolumn{4}{c}{Corr. to Output Difference} & \multicolumn{4}{c}{Label Randomization} & \multicolumn{4}{c}{Shortcut Affinity} & \multicolumn{4}{c}{Augmentation} & \multicolumn{4}{c}{Layer Monotonicity} \\
% Eval. & \multicolumn{2}{c}{Spearman} & \multicolumn{2}{c}{Spearman} & \multicolumn{2}{c}{Spearman} & \multicolumn{2}{c}{AUPRC} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{AUPRC} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{AUPRC} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{Spearman} \\
Eval. & \multicolumn{2}{c}{Spearman} & \multicolumn{2}{c}{Spearman/JSD} & \multicolumn{2}{c}{Spearman/Disagr.} & \multicolumn{2}{c}{AUPRC} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{AUPRC} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{AUPRC} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{Conformity Rate} & \multicolumn{2}{c}{Spearman} \\
Dataset & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 & MNLI & SST2 \\
\midrule
\rowcolor{Gray}2nd-Cos & -0.26$^{\phantom{**}}$ & 0.30$^{*\phantom{*}}$ & 0.16$^{\phantom{**}}$ & 0.41$^{**}$ & \textbf{0.55}$^{**}$ & -0.00$^{\phantom{**}}$ & 0.39 & 0.37 & nan & 0.64 & 0.59 & \textbf{0.55} & 0.82 & 0.84 & 0.44 & 0.40 & 0.64 & 0.64 & 0.94 & 0.96 & 0.94 & 0.97 \\
AlignCos & 0.25$^{\phantom{**}}$ & 0.02$^{\phantom{**}}$ & 0.37$^{**}$ & 0.40$^{**}$ & -0.16$^{\phantom{**}}$ & 0.15$^{\phantom{**}}$ & \textbf{1.00} & \textbf{0.99} & \textbf{1.00} & \textbf{1.00} & 0.58 & 0.45 & 0.89 & 0.79 & 0.35 & 0.45 & 0.80 & 0.63 & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.99 \\
\rowcolor{Gray}AngShape & 0.28$^{\phantom{**}}$ & -0.14$^{\phantom{**}}$ & 0.26$^{\phantom{**}}$ & 0.29$^{\phantom{**}}$ & -0.02$^{\phantom{**}}$ & 0.39$^{**}$ & 0.90 & 0.49 & 0.98 & 0.75 & \textbf{0.60} & 0.31 & \textbf{0.90} & 0.77 & 0.38 & 0.52 & 0.84 & 0.62 & 0.99 & 0.98 & \textbf{1.00} & 0.99 \\
CKA & 0.18$^{\phantom{**}}$ & -0.06$^{\phantom{**}}$ & 0.30$^{*\phantom{*}}$ & 0.39$^{**}$ & -0.01$^{\phantom{**}}$ & 0.43$^{**}$ & 0.75 & 0.59 & 0.90 & 0.78 & 0.59 & 0.26 & 0.88 & 0.67 & 0.48 & 0.61 & \textbf{0.87} & 0.68 & 0.98 & 0.98 & 0.99 & 0.96 \\
\rowcolor{Gray}ConcDiff & -0.00$^{\phantom{**}}$ & 0.12$^{\phantom{**}}$ & 0.02$^{\phantom{**}}$ & 0.05$^{\phantom{**}}$ & -0.31$^{*\phantom{*}}$ & -0.21$^{\phantom{**}}$ & \textbf{1.00} & 0.96 & \textbf{1.00} & 0.99 & 0.38 & 0.26 & 0.75 & 0.67 & 0.28 & 0.32 & 0.61 & 0.51 & 0.99 & 0.96 & 0.99 & 0.96 \\
DistCorr & 0.15$^{\phantom{**}}$ & -0.10$^{\phantom{**}}$ & 0.39$^{*\phantom{*}}$ & 0.42$^{**}$ & 0.12$^{\phantom{**}}$ & 0.44$^{**}$ & 0.75 & 0.59 & 0.89 & 0.80 & 0.58 & 0.26 & 0.88 & 0.68 & 0.45 & \textbf{0.62} & 0.85 & \textbf{0.69} & 0.96 & 0.97 & 0.97 & 0.98 \\
\rowcolor{Gray}EOS & 0.03$^{\phantom{**}}$ & -0.38$^{*\phantom{*}}$ & 0.36$^{*\phantom{*}}$ & -0.38$^{*\phantom{*}}$ & 0.01$^{\phantom{**}}$ & -0.22$^{\phantom{**}}$ & 0.62 & 0.36 & 0.88 & 0.60 & 0.57 & 0.25 & 0.85 & 0.59 & 0.27 & 0.30 & 0.71 & 0.49 & 0.98 & 0.91 & 0.99 & 0.92 \\
GULP & -0.01$^{\phantom{**}}$ & -0.36$^{*\phantom{*}}$ & 0.35$^{*\phantom{*}}$ & -0.47$^{**}$ & 0.02$^{\phantom{**}}$ & -0.27$^{\phantom{**}}$ & 0.61 & 0.28 & 0.89 & 0.54 & 0.56 & 0.25 & 0.84 & 0.65 & 0.26 & 0.33 & 0.69 & 0.47 & 0.84 & 0.78 & 0.51 & 0.45 \\
\rowcolor{Gray}HardCorr & 0.04$^{\phantom{**}}$ & -0.33$^{*\phantom{*}}$ & -0.27$^{\phantom{**}}$ & -0.19$^{\phantom{**}}$ & -0.43$^{**}$ & 0.22$^{\phantom{**}}$ & 0.75 & 0.44 & 0.90 & 0.77 & 0.55 & 0.23 & 0.82 & 0.64 & 0.24 & 0.34 & 0.67 & 0.49 & \textbf{1.00} & 0.99 & \textbf{1.00} & 0.99 \\
IMD & -0.26$^{\phantom{**}}$ & -0.06$^{\phantom{**}}$ & -0.39$^{**}$ & 0.13$^{\phantom{**}}$ & -0.06$^{\phantom{**}}$ & 0.35$^{*\phantom{*}}$ & 0.73 & 0.47 & 0.92 & 0.79 & 0.53 & 0.34 & 0.82 & 0.72 & 0.43 & 0.30 & 0.75 & 0.47 & 0.68 & 0.64 & 0.44 & 0.54 \\
\rowcolor{Gray}Jaccard & -0.21$^{\phantom{**}}$ & 0.17$^{\phantom{**}}$ & 0.13$^{\phantom{**}}$ & 0.46$^{**}$ & 0.17$^{\phantom{**}}$ & 0.09$^{\phantom{**}}$ & 0.69 & 0.35 & 0.84 & 0.69 & 0.56 & \textbf{0.55} & 0.81 & \textbf{0.86} & 0.35 & 0.39 & 0.74 & 0.61 & 0.95 & 0.94 & 0.96 & 0.96 \\
LinReg & 0.18$^{\phantom{**}}$ & -0.38$^{**}$ & 0.28$^{**}$ & -0.14$^{\phantom{**}}$ & -0.03$^{\phantom{**}}$ & 0.21$^{\phantom{**}}$ & 0.57 & 0.40 & 0.85 & 0.57 & 0.46 & 0.37 & 0.85 & 0.74 & 0.24 & 0.40 & 0.66 & 0.55 & 0.83 & 0.93 & 0.66 & 0.90 \\
\rowcolor{Gray}MagDiff & 0.22$^{\phantom{**}}$ & -0.13$^{\phantom{**}}$ & 0.01$^{\phantom{**}}$ & 0.02$^{\phantom{**}}$ & -0.03$^{\phantom{**}}$ & -0.06$^{\phantom{**}}$ & 0.33 & 0.38 & 0.75 & 0.69 & 0.48 & 0.35 & 0.81 & 0.73 & 0.16 & 0.31 & 0.45 & 0.46 & 0.64 & 0.62 & 0.52 & 0.48 \\
OrthProc & 0.28$^{\phantom{**}}$ & -0.14$^{\phantom{**}}$ & 0.26$^{\phantom{**}}$ & 0.29$^{\phantom{**}}$ & -0.02$^{\phantom{**}}$ & 0.39$^{**}$ & 0.90 & 0.49 & 0.98 & 0.75 & \textbf{0.60} & 0.31 & \textbf{0.90} & 0.77 & 0.38 & 0.52 & 0.84 & 0.62 & 0.98 & 0.98 & 0.99 & 0.99 \\
\rowcolor{Gray}PWCCA & 0.01$^{\phantom{**}}$ & -0.33$^{*\phantom{*}}$ & 0.22$^{\phantom{**}}$ & -0.39$^{*\phantom{*}}$ & -0.37$^{*\phantom{*}}$ & -0.28$^{\phantom{**}}$ & 0.65 & 0.27 & 0.91 & 0.48 & 0.56 & 0.35 & 0.86 & 0.69 & 0.18 & 0.35 & 0.49 & 0.38 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
PermProc & 0.09$^{\phantom{**}}$ & -0.09$^{\phantom{**}}$ & -0.06$^{\phantom{**}}$ & -0.13$^{\phantom{**}}$ & -0.30$^{\phantom{**}}$ & 0.04$^{\phantom{**}}$ & 0.44 & 0.45 & 0.68 & 0.73 & 0.52 & 0.46 & 0.82 & 0.78 & 0.18 & 0.31 & 0.49 & 0.44 & 0.80 & 0.83 & 0.73 & 0.75 \\
\rowcolor{Gray}ProcDist & 0.28$^{\phantom{**}}$ & 0.10$^{\phantom{**}}$ & 0.07$^{\phantom{**}}$ & 0.40$^{**}$ & -0.38$^{**}$ & 0.27$^{\phantom{**}}$ & 0.98 & 0.86 & 0.99 & 0.95 & 0.54 & 0.43 & 0.87 & 0.77 & 0.32 & 0.43 & 0.73 & 0.64 & 0.96 & 0.97 & 0.92 & 0.89 \\
RSA & 0.00$^{\phantom{**}}$ & -0.23$^{\phantom{**}}$ & 0.27$^{\phantom{**}}$ & 0.34$^{*\phantom{*}}$ & 0.19$^{\phantom{**}}$ & \textbf{0.52}$^{**}$ & 0.46 & 0.48 & 0.64 & 0.73 & 0.58 & 0.36 & 0.87 & 0.68 & 0.49 & 0.61 & 0.86 & 0.68 & 0.99 & 0.95 & \textbf{1.00} & 0.96 \\
\rowcolor{Gray}RSMDiff & 0.30$^{*\phantom{*}}$ & 0.20$^{\phantom{**}}$ & -0.18$^{\phantom{**}}$ & 0.35$^{*\phantom{*}}$ & -0.19$^{\phantom{**}}$ & -0.03$^{\phantom{**}}$ & 0.52 & 0.91 & 0.67 & 0.97 & 0.28 & 0.34 & 0.66 & 0.69 & 0.35 & 0.34 & 0.66 & 0.58 & 0.94 & 0.95 & 0.84 & 0.84 \\
RankSim & -0.09$^{\phantom{**}}$ & 0.14$^{\phantom{**}}$ & 0.08$^{\phantom{**}}$ & \textbf{0.49}$^{**}$ & 0.05$^{\phantom{**}}$ & 0.11$^{\phantom{**}}$ & 0.63 & 0.34 & 0.82 & 0.63 & 0.58 & \textbf{0.55} & 0.82 & \textbf{0.86} & 0.33 & 0.36 & 0.71 & 0.57 & 0.93 & 0.94 & 0.90 & 0.96 \\
\rowcolor{Gray}SVCCA & \textbf{0.32}$^{*\phantom{*}}$ & -0.08$^{\phantom{**}}$ & \textbf{0.47}$^{**}$ & 0.37$^{*\phantom{*}}$ & 0.00$^{\phantom{**}}$ & 0.40$^{**}$ & 0.69 & 0.64 & 0.86 & 0.80 & 0.42 & 0.25 & 0.78 & 0.62 & 0.44 & 0.61 & 0.77 & 0.68 & 0.91 & 0.88 & 0.91 & 0.64 \\
SoftCorr & 0.11$^{\phantom{**}}$ & -0.33$^{*\phantom{*}}$ & -0.23$^{\phantom{**}}$ & -0.18$^{\phantom{**}}$ & -0.42$^{**}$ & 0.24$^{\phantom{**}}$ & 0.75 & 0.48 & 0.92 & 0.80 & 0.55 & 0.22 & 0.82 & 0.55 & 0.28 & 0.41 & 0.72 & 0.52 & 0.98 & 0.96 & 0.99 & 0.95 \\
\rowcolor{Gray}UnifDiff & 0.14$^{\phantom{**}}$ & \textbf{0.35}$^{*\phantom{*}}$ & -0.02$^{\phantom{**}}$ & 0.35$^{*\phantom{*}}$ & -0.14$^{\phantom{**}}$ & -0.10$^{\phantom{**}}$ & 0.76 & 0.60 & 0.91 & 0.86 & 0.40 & 0.35 & 0.69 & 0.55 & \textbf{0.61} & 0.33 & 0.84 & 0.46 & 0.94 & 0.85 & 0.81 & 0.77 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/runtimes.tex <==

\begin{table}[hb]
\centering
    \caption{\textit{Runtime of the similarity metrics in seconds, averaged over all comparisons for Test 6 (Layer Monotonicity)}. Since embedding dimensions and the number of inputs varies for different datasets, and we aggregate across datasets within each domain, the runtime should be interpreted as a broad estimate of the runtime to be expected.}
    \label{tab:runtimes}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|rrr|r|rrrrrrr}
\toprule
Modality & \multicolumn{3}{c|}{Graph} & Lang. & \multicolumn{7}{c}{Vision} \\
Architecture & GAT & GCN & GraphSAGE & BERT & ResNet18 & ResNet34 & ResNet101 & VGG11 & VGG19 & ViT B32 & ViT L32 \\
\midrule
2nd-Cos & 3.150 & 3.180 & 3.000 & 7.360 & 2.800 & 2.790 & 4.510 & 3.210 & 3.600 & 2.650 & 4.060 \\
\rowcolor{Gray}AlignCos & 0.060 & 0.060 & 0.060 & 0.570 & 0.310 & 0.270 & 4.890 & 0.400 & 0.380 & 0.410 & 1.220 \\
AngShape & 0.040 & 0.040 & 0.040 & 0.580 & 0.320 & 0.300 & 5.560 & 0.430 & 0.360 & 0.490 & 1.440 \\
\rowcolor{Gray}CKA & 0.030 & 0.030 & 0.030 & 0.170 & 3.040 & 1.380 & 25.180 & 7.740 & 7.090 & 0.300 & 0.830 \\
ConcDiff & 0.010 & 0.010 & 0.010 & 0.140 & 0.100 & 0.120 & 0.950 & 0.270 & 0.200 & 0.030 & 0.040 \\
\rowcolor{Gray}DistCorr & 1.750 & 1.830 & 1.710 & 4.600 & 4.630 & 3.200 & 25.150 & 10.930 & 7.770 & 2.260 & 3.650 \\
EOS & 15.510 & 16.840 & 15.220 & 6.140 & 11.930 & 13.990 & 37.520 & 24.400 & 14.140 & 15.830 & 21.750 \\
\rowcolor{Gray}GULP & 0.040 & 0.040 & 0.040 & 0.710 & 0.400 & 0.380 & 9.000 & 0.540 & 0.530 & 0.770 & 2.270 \\
HardCorr & 0.020 & 0.020 & 0.020 & 0.240 & 0.160 & 0.160 & 1.710 & 0.270 & 0.220 & 0.170 & 0.360 \\
\rowcolor{Gray}IMD & 157.900 & 157.840 & 159.180 & 215.070 & 367.270 & 459.580 & 297.490 & 581.300 & 434.110 & 296.040 & 275.370 \\
Jaccard & 2.530 & 2.550 & 2.400 & 8.190 & 1.970 & 2.000 & 2.840 & 2.200 & 2.450 & 1.750 & 2.530 \\
\rowcolor{Gray}LinReg & 0.040 & 0.080 & 0.040 & 0.600 & 1.070 & 0.450 & 16.100 & 0.610 & 0.530 & 1.680 & 4.180 \\
MagDiff & 0.000 & 0.000 & 0.000 & 0.010 & 0.010 & 0.010 & 0.100 & 0.020 & 0.020 & 0.000 & 0.010 \\
\rowcolor{Gray}OrthProc & 0.020 & 0.020 & 0.020 & 0.540 & 0.240 & 0.220 & 4.400 & 0.330 & 0.250 & 0.310 & 1.010 \\
PWCCA & NaN & NaN & NaN & 2.040 & 1.650 & 1.790 & 36.730 & 1.780 & 2.860 & 2.860 & 7.660 \\
\rowcolor{Gray}PermProc & 0.020 & 0.020 & 0.020 & 0.370 & 0.200 & 0.190 & 4.140 & 0.340 & 0.270 & 0.290 & 0.500 \\
ProcDist & 0.020 & 0.020 & 0.020 & 0.510 & 0.220 & 0.200 & 4.430 & 0.310 & 0.240 & 0.310 & 0.990 \\
\rowcolor{Gray}RSA & 17.080 & 16.860 & 16.020 & 40.570 & 10.660 & 9.360 & 17.650 & 14.420 & 14.210 & 8.670 & 11.990 \\
RSMDiff & 106.090 & 106.290 & 105.870 & 108.980 & 52.640 & 61.200 & 77.710 & 97.060 & 62.710 & 62.540 & 56.270 \\
\rowcolor{Gray}RankSim & 2.650 & 2.710 & 2.450 & 8.430 & 2.220 & 2.280 & 3.200 & 2.560 & 2.700 & 2.010 & 3.050 \\
SVCCA & 0.420 & 0.460 & 0.420 & 4.740 & 2.500 & 2.060 & 24.250 & 3.570 & 3.280 & 3.190 & 9.730 \\
\rowcolor{Gray}SoftCorr & 0.020 & 0.020 & 0.020 & 0.110 & 0.130 & 0.130 & 1.270 & 0.250 & 0.180 & 0.140 & 0.290 \\
UnifDiff & 8.110 & 9.210 & 7.450 & 148.110 & 10.100 & 9.710 & 33.760 & 14.960 & 12.520 & 13.940 & 22.480 \\
\bottomrule
\end{tabular}}

\end{table}

==> tables/scores_agg_per_test.tex <==
\begin{table}[t]
\caption{Vision}
\label{tab:results_agg_per_test}
\resizebox{0.95\linewidth}{!}{\begin{tabular}{lrrrrrrr}
\toprule
Type & \multicolumn{3}{r}{Grounding by Prediction} & \multicolumn{4}{r}{Grounding by Design} \\
Scenario & Acc Corr. & JSD Corr. & Disagr. Corr. & Random Labels & Shortcuts & Augmentation & Layer Mono. \\
\midrule
\rowcolor{Gray}2nd-Cos & 15.7 & 13.1 & 11.9 & 17.3 & \textbf{5.8} & 6.3 & 6.6 \\
AlignCos & 16.1 & 12.0 & 8.4 & 13.2 & \textbf{5.8} & \textbf{4.7} & 11.8 \\
\rowcolor{Gray}AngShape & 8.8 & 9.1 & 12.4 & 8.9 & 6.1 & 9.9 & 8.3 \\
CKA & 10.1 & 11.0 & 8.7 & 6.9 & \textbf{5.8} & 8.6 & 6.6 \\
\rowcolor{Gray}ConcDiff & 13.1 & 17.6 & 17.0 & 7.0 & 20.6 & 12.6 & 20.1 \\
DistCorr & 12.7 & 10.4 & 9.0 & 6.3 & \textbf{5.8} & 10.8 & 6.5 \\
\rowcolor{Gray}EOS & 12.0 & 11.4 & 14.6 & 14.9 & 10.8 & 7.3 & \textbf{5.0} \\
GULP & 11.4 & 10.1 & 14.0 & 16.6 & 9.1 & 7.1 & 9.4 \\
\rowcolor{Gray}HardCorr & 9.7 & 12.6 & 13.3 & 12.4 & 12.0 & 17.4 & 11.8 \\
IMD & 14.1 & 9.3 & 7.0 & 5.7 & 15.9 & 13.9 & 21.0 \\
\rowcolor{Gray}Jaccard & 14.1 & \textbf{5.7} & 6.7 & 8.7 & 7.0 & 6.3 & 7.5 \\
LinReg & 9.3 & 7.9 & 11.0 & 21.5 & 9.3 & 7.7 & 9.0 \\
\rowcolor{Gray}MagDiff & 14.0 & 19.3 & 15.9 & 5.8 & 23.0 & 15.9 & 17.9 \\
OrthProc & 8.8 & 9.4 & 12.4 & 8.9 & 6.1 & 9.9 & 8.3 \\
\rowcolor{Gray}PWCCA & 12.6 & 11.3 & 15.1 & nan & 11.6 & 12.4 & 13.1 \\
PermProc & 11.6 & 10.6 & 9.1 & 16.2 & 17.6 & 18.3 & 14.8 \\
\rowcolor{Gray}ProcDist & 6.9 & 8.6 & 12.7 & 12.4 & 6.1 & 9.3 & 14.3 \\
RSA & 14.6 & 15.9 & 9.7 & 10.9 & \textbf{5.8} & 11.7 & 8.3 \\
\rowcolor{Gray}RSMDiff & 12.1 & 16.9 & 15.0 & \textbf{5.5} & 19.6 & 17.6 & 16.9 \\
RankSim & \textbf{6.4} & 12.3 & 15.6 & 7.7 & 9.2 & 9.9 & 7.7 \\
\rowcolor{Gray}SVCCA & 12.9 & 10.3 & 8.0 & 11.6 & 19.0 & 18.4 & 16.8 \\
SoftCorr & 10.6 & 11.9 & 12.6 & 14.9 & 13.6 & 17.0 & 13.2 \\
\rowcolor{Gray}UnifDiff & 12.3 & 15.0 & \textbf{6.7} & 19.3 & 18.8 & 23.0 & 18.3 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\caption{Graph}
\label{tab:results_agg_per_test}
\resizebox{0.95\linewidth}{!}{\begin{tabular}{lrrrrrrr}
\toprule
Type & \multicolumn{3}{r}{Grounding by Prediction} & \multicolumn{4}{r}{Grounding by Design} \\
Scenario & Acc Corr. & JSD Corr. & Disagr. Corr. & Random Labels & Shortcuts & Augmentation & Layer Mono. \\
\midrule
\rowcolor{Gray}2nd-Cos & 14.0 & 9.3 & 10.4 & 6.8 & \textbf{4.5} & \textbf{3.8} & 12.1 \\
AlignCos & 11.8 & 12.5 & 13.4 & 9.0 & 7.6 & 11.7 & 17.6 \\
\rowcolor{Gray}AngShape & 12.1 & 8.2 & 8.0 & 11.1 & 8.9 & 11.1 & 12.2 \\
CKA & 10.7 & 10.7 & 11.0 & 7.7 & 10.0 & 10.2 & 15.0 \\
\rowcolor{Gray}ConcDiff & 14.2 & 16.6 & 17.4 & 12.9 & 17.8 & 18.1 & 28.0 \\
DistCorr & 9.0 & 9.5 & 9.6 & 8.2 & 9.1 & 7.0 & 14.1 \\
\rowcolor{Gray}EOS & \textbf{7.7} & 13.3 & 13.8 & 19.6 & 14.3 & 14.1 & \textbf{10.1} \\
GULP & 11.8 & 12.4 & 14.2 & 19.9 & 17.1 & 15.9 & 13.1 \\
\rowcolor{Gray}HardCorr & 10.3 & 9.5 & 8.9 & 11.4 & 14.8 & 13.6 & 21.4 \\
IMD & 13.5 & 17.0 & 17.9 & 8.4 & 10.2 & 13.3 & 10.3 \\
\rowcolor{Gray}Jaccard & 15.4 & 7.5 & 8.6 & 13.3 & 6.5 & 4.7 & 10.9 \\
LinReg & 14.4 & 10.1 & 11.1 & 12.8 & 10.5 & 11.3 & 12.5 \\
\rowcolor{Gray}MagDiff & 11.0 & 16.9 & 17.4 & 17.3 & 18.0 & 16.1 & 24.6 \\
OrthProc & 11.9 & 8.3 & 8.1 & 11.1 & 8.9 & 11.1 & 12.2 \\
\rowcolor{Gray}PWCCA & 14.8 & 16.5 & 13.2 & nan & nan & nan & 14.1 \\
PermProc & 8.4 & 14.6 & 12.0 & 10.9 & 17.6 & 13.4 & 16.2 \\
\rowcolor{Gray}ProcDist & 11.4 & 13.9 & 12.8 & 7.9 & 8.6 & 8.0 & 12.5 \\
RSA & 10.6 & \textbf{6.4} & \textbf{5.0} & 11.1 & 10.0 & 13.4 & 19.1 \\
\rowcolor{Gray}RSMDiff & 12.5 & 17.6 & 15.3 & \textbf{5.7} & 8.1 & 5.5 & 12.8 \\
RankSim & 13.4 & 8.0 & 9.3 & 11.3 & 7.5 & 6.4 & 10.7 \\
\rowcolor{Gray}SVCCA & 16.0 & 13.3 & 14.3 & 11.2 & 15.0 & 15.2 & 26.5 \\
SoftCorr & 8.7 & 9.2 & 8.4 & 12.3 & 13.2 & 14.7 & 19.8 \\
\rowcolor{Gray}UnifDiff & 14.3 & 15.0 & 14.8 & 13.1 & 14.9 & 14.4 & 24.9 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\caption{Language}
\label{tab:results_agg_per_test}
\resizebox{0.95\linewidth}{!}{\begin{tabular}{lrrrrrrr}
\toprule
Type & \multicolumn{3}{r}{Grounding by Prediction} & \multicolumn{4}{r}{Grounding by Design} \\
Scenario & Acc Corr. & JSD Corr. & Disagr. Corr. & Random Labels & Shortcuts & Augmentation & Layer Mono. \\
\midrule
\rowcolor{Gray}2nd-Cos & 12.0 & 8.0 & 8.5 & 20.0 & \textbf{3.0} & 7.5 & 6.6 \\
AlignCos & 7.0 & 4.0 & 14.0 & \textbf{1.2} & 5.5 & 9.0 & 3.4 \\
\rowcolor{Gray}AngShape & 10.0 & 11.0 & 8.0 & 7.0 & 8.0 & 7.0 & 4.9 \\
CKA & 9.5 & 6.5 & 6.0 & 8.0 & 10.5 & 3.0 & 8.6 \\
\rowcolor{Gray}ConcDiff & 12.0 & 15.5 & 19.5 & 1.8 & 20.0 & 17.0 & 7.0 \\
DistCorr & 11.5 & \textbf{2.5} & 3.0 & 8.0 & 10.5 & 2.5 & 8.2 \\
\rowcolor{Gray}EOS & 18.5 & 12.5 & 14.0 & 17.5 & 15.0 & 19.5 & 10.2 \\
GULP & 20.0 & 14.0 & 14.0 & 19.5 & 15.5 & 17.5 & 21.0 \\
\rowcolor{Gray}HardCorr & 17.0 & 21.0 & 16.5 & 12.5 & 18.0 & 17.0 & 3.9 \\
IMD & 16.0 & 18.5 & 10.5 & 12.0 & 14.5 & 15.0 & 21.2 \\
\rowcolor{Gray}Jaccard & 12.5 & 7.5 & 8.5 & 16.5 & 5.5 & 12.0 & 10.2 \\
LinReg & 15.5 & 12.5 & 12.0 & 17.0 & 13.0 & 15.5 & 15.2 \\
\rowcolor{Gray}MagDiff & 10.5 & 16.5 & 15.0 & 20.0 & 14.0 & 22.0 & 20.8 \\
OrthProc & 10.0 & 11.0 & 8.0 & 7.0 & 8.0 & 7.0 & 6.7 \\
\rowcolor{Gray}PWCCA & 17.5 & 16.5 & 21.5 & 18.5 & 10.5 & 17.5 & \textbf{2.5} \\
PermProc & 12.5 & 18.0 & 16.5 & 17.5 & 10.5 & 21.0 & 18.6 \\
\rowcolor{Gray}ProcDist & 5.0 & 10.5 & 14.5 & 3.5 & 10.5 & 11.0 & 14.0 \\
RSA & 17.0 & 9.5 & \textbf{1.5} & 16.0 & 7.5 & \textbf{2.0} & 4.7 \\
\rowcolor{Gray}RSMDiff & \textbf{2.5} & 15.0 & 17.0 & 11.0 & 17.5 & 13.0 & 16.2 \\
RankSim & 12.5 & 7.5 & 9.0 & 18.0 & 5.0 & 13.0 & 12.3 \\
\rowcolor{Gray}SVCCA & 6.0 & 4.5 & 6.0 & 8.5 & 19.5 & 5.0 & 16.5 \\
SoftCorr & 15.0 & 20.0 & 15.5 & 9.0 & 18.0 & 12.5 & 9.5 \\
\rowcolor{Gray}UnifDiff & 6.0 & 13.5 & 17.0 & 6.0 & 16.0 & 9.5 & 17.4 \\
\bottomrule
\end{tabular}}
\end{table}

==> tables/vision_outputcorr_JSD.tex <==
\begin{table}
\caption{Correlation between functional similarity measure JSD and similarity measure. Models Trained on C10.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
architecture & \multicolumn{3}{c}{ResNet18} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{VGG11} \\
quality measure & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr \\
similarity measure &  &  &  &  &  &  &  &  &  \\
\midrule
\textbf{CKA} & 0.067 & -0.042 & 0.091 & 0.289 & 0.485 & 0.358 & -0.067 & -0.381 & -0.261 \\
\textbf{DistanceCorrelation} & 0.111 & -0.170 & 0.103 & 0.244 & 0.364 & 0.309 & -0.333 & -0.597 & -0.455 \\
\textbf{HardCorrelationMatch} & -0.378 & -0.552 & -0.661 & -0.200 & -0.110 & -0.115 & 0.111 & 0.099 & 0.127 \\
\textbf{JaccardSimilarity} & 0.156 & -0.032 & 0.212 & -0.156 & 0.030 & -0.188 & 0.200 & 0.178 & 0.236 \\
\textbf{MagnitudeDifference} & 0.422 & 0.470 & 0.564 & 0.289 & 0.269 & 0.382 & 0.111 & 0.135 & 0.067 \\
\textbf{PermutationProcrustes} & 0.200 & 0.252 & 0.321 & -0.067 & -0.033 & -0.115 & 0.244 & 0.425 & 0.333 \\
\textbf{RSA} & 0.156 & 0.276 & 0.188 & 0.022 & 0.227 & 0.018 & 0.067 & -0.061 & 0.115 \\
\textbf{RankSimilarity} & -0.022 & -0.073 & -0.006 & 0.111 & 0.286 & 0.042 & -0.022 & -0.040 & -0.030 \\
\textbf{SecondOrderCosineSimilarity} & 0.111 & 0.001 & 0.115 & 0.289 & 0.380 & 0.406 & 0.289 & 0.206 & 0.297 \\
\textbf{SoftCorrelationMatch} & -0.422 & -0.565 & -0.685 & 0.022 & -0.036 & 0.042 & -0.067 & 0.056 & -0.055 \\
\bottomrule
\end{tabular}}
\end{table}
\begin{table}
\caption{Correlation between functional similarity measure JSD and similarity measure. Models Trained in Gauss Noise Setting.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
architecture & \multicolumn{3}{c}{ResNet18} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{VGG11} \\
quality measure & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr \\
similarity measure &  &  &  &  &  &  &  &  &  \\
\midrule
\textbf{CKA} & -0.886 & -0.990 & -0.979 & -0.908 & -0.990 & -0.988 & -0.838 & -0.964 & -0.957 \\
\textbf{DistanceCorrelation} & -0.923 & -0.987 & -0.991 & -0.879 & -0.977 & -0.980 & -0.884 & -0.976 & -0.976 \\
\textbf{HardCorrelationMatch} & -0.911 & -0.993 & -0.990 & -0.903 & -0.993 & -0.988 & -0.372 & -0.545 & -0.530 \\
\textbf{JaccardSimilarity} & -0.589 & -0.857 & -0.797 & -0.647 & -0.880 & -0.845 & -0.494 & -0.719 & -0.702 \\
\textbf{MagnitudeDifference} & 0.766 & 0.906 & 0.904 & 0.002 & -0.017 & -0.005 & 0.740 & 0.899 & 0.897 \\
\textbf{PermutationProcrustes} & 0.787 & 0.958 & 0.946 & 0.761 & 0.936 & 0.934 & 0.512 & 0.711 & 0.701 \\
\textbf{RSA} & -0.616 & -0.887 & -0.832 & -0.667 & -0.889 & -0.863 & -0.524 & -0.798 & -0.722 \\
\textbf{RankSimilarity} & -0.575 & -0.851 & -0.786 & -0.628 & -0.858 & -0.820 & -0.487 & -0.722 & -0.698 \\
\textbf{SecondOrderCosineSimilarity} & -0.340 & -0.555 & -0.506 & -0.406 & -0.640 & -0.578 & -0.317 & -0.553 & -0.469 \\
\textbf{SoftCorrelationMatch} & -0.863 & -0.985 & -0.975 & -0.885 & -0.994 & -0.983 & -0.400 & -0.585 & -0.569 \\
\bottomrule
\end{tabular}}
\end{table}
\begin{table}
\caption{Correlation between functional similarity measure JSD and similarity measure. Models Trained in Shortcut Setting.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
architecture & \multicolumn{3}{c}{ResNet18} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{VGG11} \\
quality measure & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr \\
similarity measure &  &  &  &  &  &  &  &  &  \\
\midrule
\textbf{CKA} & -0.737 & -0.988 & -0.860 & -0.771 & -0.995 & -0.877 & -0.886 & -0.993 & -0.973 \\
\textbf{DistanceCorrelation} & -0.774 & -0.992 & -0.880 & -0.804 & -0.996 & -0.892 & -0.888 & -0.992 & -0.973 \\
\textbf{HardCorrelationMatch} & -0.670 & -0.934 & -0.822 & -0.745 & -0.966 & -0.865 & -0.606 & -0.818 & -0.802 \\
\textbf{JaccardSimilarity} & -0.709 & -0.528 & -0.855 & -0.667 & -0.530 & -0.817 & -0.821 & -0.645 & -0.945 \\
\textbf{MagnitudeDifference} & 0.052 & 0.053 & 0.107 & 0.596 & 0.934 & 0.777 & 0.730 & 0.988 & 0.907 \\
\textbf{PermutationProcrustes} & 0.657 & 0.935 & 0.819 & 0.671 & 0.976 & 0.811 & 0.737 & 0.942 & 0.892 \\
\textbf{RSA} & -0.631 & -0.944 & -0.787 & -0.626 & -0.972 & -0.779 & -0.823 & -0.979 & -0.946 \\
\textbf{RankSimilarity} & -0.660 & -0.621 & -0.816 & -0.607 & -0.610 & -0.764 & -0.800 & -0.695 & -0.935 \\
\textbf{SecondOrderCosineSimilarity} & -0.653 & -0.980 & -0.806 & -0.675 & -0.985 & -0.818 & -0.830 & -0.990 & -0.936 \\
\textbf{SoftCorrelationMatch} & -0.670 & -0.931 & -0.817 & -0.749 & -0.964 & -0.866 & -0.605 & -0.800 & -0.806 \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/vision_outputcorr_disagreement.tex <==
\begin{table}
\caption{Correlation between functional similarity measure Disagreement and similarity measure. Models Trained on C10.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
architecture & \multicolumn{3}{c}{ResNet18} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{VGG11} \\
quality measure & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr \\
similarity measure &  &  &  &  &  &  &  &  &  \\
\midrule
\textbf{CKA} & 0.405 & 0.633 & 0.529 & -0.067 & 0.079 & 0.067 & 0.022 & 0.056 & 0.055 \\
\textbf{DistanceCorrelation} & 0.449 & 0.621 & 0.578 & -0.022 & 0.128 & 0.079 & 0.111 & 0.016 & 0.248 \\
\textbf{HardCorrelationMatch} & -0.315 & -0.420 & -0.365 & -0.200 & -0.373 & -0.321 & 0.289 & 0.617 & 0.394 \\
\textbf{JaccardSimilarity} & 0.494 & 0.551 & 0.571 & -0.067 & 0.090 & -0.067 & 0.467 & 0.720 & 0.612 \\
\textbf{MagnitudeDifference} & 0.180 & 0.236 & 0.219 & 0.556 & 0.696 & 0.758 & 0.022 & 0.023 & -0.006 \\
\textbf{PermutationProcrustes} & 0.494 & 0.522 & 0.614 & 0.200 & 0.498 & 0.394 & 0.067 & -0.095 & 0.067 \\
\textbf{RSA} & 0.315 & 0.579 & 0.511 & -0.244 & -0.339 & -0.370 & 0.067 & -0.044 & 0.091 \\
\textbf{RankSimilarity} & 0.225 & 0.416 & 0.347 & -0.156 & -0.158 & -0.212 & 0.244 & 0.514 & 0.333 \\
\textbf{SecondOrderCosineSimilarity} & 0.270 & 0.597 & 0.353 & 0.022 & 0.181 & 0.164 & 0.289 & 0.562 & 0.479 \\
\textbf{SoftCorrelationMatch} & -0.270 & -0.477 & -0.340 & -0.156 & -0.442 & -0.370 & 0.378 & 0.673 & 0.539 \\
\bottomrule
\end{tabular}}
\end{table}
\begin{table}
\caption{Correlation between functional similarity measure Disagreement and similarity measure. Models Trained in Gauss Noise Setting.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
architecture & \multicolumn{3}{c}{ResNet18} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{VGG11} \\
quality measure & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr \\
similarity measure &  &  &  &  &  &  &  &  &  \\
\midrule
\textbf{CKA} & -0.842 & -0.970 & -0.964 & -0.890 & -0.986 & -0.983 & -0.785 & -0.941 & -0.927 \\
\textbf{DistanceCorrelation} & -0.868 & -0.967 & -0.975 & -0.862 & -0.971 & -0.975 & -0.829 & -0.956 & -0.953 \\
\textbf{HardCorrelationMatch} & -0.887 & -0.990 & -0.984 & -0.892 & -0.991 & -0.985 & -0.363 & -0.538 & -0.518 \\
\textbf{JaccardSimilarity} & -0.547 & -0.805 & -0.757 & -0.639 & -0.871 & -0.834 & -0.436 & -0.661 & -0.633 \\
\textbf{MagnitudeDifference} & 0.765 & 0.884 & 0.895 & -0.003 & -0.027 & -0.011 & 0.742 & 0.892 & 0.890 \\
\textbf{PermutationProcrustes} & 0.824 & 0.979 & 0.963 & 0.757 & 0.930 & 0.930 & 0.543 & 0.741 & 0.736 \\
\textbf{RSA} & -0.567 & -0.832 & -0.791 & -0.651 & -0.880 & -0.851 & -0.476 & -0.749 & -0.660 \\
\textbf{RankSimilarity} & -0.536 & -0.796 & -0.746 & -0.619 & -0.849 & -0.809 & -0.433 & -0.663 & -0.629 \\
\textbf{SecondOrderCosineSimilarity} & -0.292 & -0.464 & -0.451 & -0.395 & -0.628 & -0.562 & -0.261 & -0.485 & -0.390 \\
\textbf{SoftCorrelationMatch} & -0.888 & -0.993 & -0.983 & -0.877 & -0.991 & -0.981 & -0.390 & -0.578 & -0.555 \\
\bottomrule
\end{tabular}}
\end{table}
\begin{table}
\caption{Correlation between functional similarity measure Disagreement and similarity measure. Models Trained in Shortcut Setting.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
architecture & \multicolumn{3}{c}{ResNet18} & \multicolumn{3}{c}{ResNet34} & \multicolumn{3}{c}{VGG11} \\
quality measure & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr & kendalltau & pearsonr & spearmanr \\
similarity measure &  &  &  &  &  &  &  &  &  \\
\midrule
\textbf{CKA} & -0.703 & -0.987 & -0.843 & -0.744 & -0.995 & -0.869 & -0.869 & -0.992 & -0.970 \\
\textbf{DistanceCorrelation} & -0.739 & -0.992 & -0.864 & -0.777 & -0.996 & -0.885 & -0.869 & -0.992 & -0.970 \\
\textbf{HardCorrelationMatch} & -0.645 & -0.930 & -0.805 & -0.724 & -0.964 & -0.858 & -0.597 & -0.815 & -0.796 \\
\textbf{JaccardSimilarity} & -0.683 & -0.521 & -0.839 & -0.644 & -0.527 & -0.808 & -0.812 & -0.637 & -0.943 \\
\textbf{MagnitudeDifference} & 0.035 & 0.047 & 0.083 & 0.587 & 0.933 & 0.770 & 0.732 & 0.987 & 0.907 \\
\textbf{PermutationProcrustes} & 0.640 & 0.932 & 0.806 & 0.648 & 0.974 & 0.802 & 0.735 & 0.939 & 0.891 \\
\textbf{RSA} & -0.599 & -0.941 & -0.769 & -0.602 & -0.971 & -0.769 & -0.807 & -0.977 & -0.942 \\
\textbf{RankSimilarity} & -0.633 & -0.614 & -0.798 & -0.585 & -0.606 & -0.754 & -0.789 & -0.687 & -0.932 \\
\textbf{SecondOrderCosineSimilarity} & -0.625 & -0.978 & -0.787 & -0.654 & -0.984 & -0.810 & -0.814 & -0.988 & -0.933 \\
\textbf{SoftCorrelationMatch} & -0.640 & -0.928 & -0.799 & -0.732 & -0.961 & -0.860 & -0.593 & -0.795 & -0.797 \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/vision_shortcut_similarity.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
identifier & \multicolumn{6}{c}{Shortcut ColorDot} \\
quality measure & violation rate & AUPRC & violation rate & AUPRC & violation rate & AUPRC \\
architecture & ResNet18 & ResNet18 & ResNet34 & ResNet34 & VGG11 & VGG11 \\
similarity measure &  &  &  &  &  &  \\
\midrule
CKA & 0.000000 & 1.000000 & 0.000000 & 1.000000 & 0.000000 & 1.000000 \\
DistanceCorrelation & 0.000000 & 1.000000 & 0.000000 & 1.000000 & 0.000000 & 1.000000 \\
HardCorrelationMatch & 0.000000 & 1.000000 & 0.000000 & 1.000000 & 0.193200 & 0.418010 \\
JaccardSimilarity & 0.000000 & 1.000000 & 0.000000 & 1.000000 & 0.000000 & 1.000000 \\
MagnitudeDifference & 0.054600 & 0.722076 & 0.096600 & 0.467888 & 0.116000 & 0.531874 \\
PermutationProcrustes & 0.000000 & 1.000000 & 0.001800 & 0.989111 & 0.067400 & 0.763045 \\
RSA & 0.000000 & 1.000000 & 0.001200 & 0.990952 & 0.000000 & 1.000000 \\
RankSimilarity & 0.000000 & 1.000000 & 0.000000 & 1.000000 & 0.000000 & 1.000000 \\
SecondOrderCosineSimilarity & 0.003400 & 0.977657 & 0.000000 & 1.000000 & 0.000000 & 1.000000 \\
SoftCorrelationMatch & 0.000000 & 1.000000 & 0.000000 & 1.000000 & 0.181200 & 0.465816 \\
\bottomrule
\end{tabular}}
\end{table}
